TigerLily: Finding drug interactions in silico with the Graph

Tigerlily is a TigerGraph based system designed to solve the drug interaction prediction task. In this machine learning task, we want to predict whether two drugs have an adverse interaction. Our framework allows us to solve this highly relevant real-world problem using graph mining techniques in these steps: (a) Using PyTigergraph we create a heterogeneous biological graph of drugs and proteins. (b) We calculate the personalized PageRank scores of drug nodes in the TigerGraph Cloud. (c) We embed the nodes using sparse non-negative matrix factorization of the personalized PageRank matrix. (d) Using the node embeddings we train a gradient boosting based drug interaction predictor.

==> algorithms/batching_algorithm.tex <==
	\begin{algorithm}[h!]
{\small		\DontPrintSemicolon
		\SetAlgoLined
		\KwData{$\mathcal{B}$ -- Batch of (drug A, drug B, cell line, label) tuples.\\
		$\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\mathcal{G}$ -- Graph of interest.\\
		$\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,s$ -- Sample size for multi-scale approximation.\\
		}
		\KwResult{$\mathcal{L}$ -- Average loss on batch $\mathcal{B}$.}
$\mathcal{L}\leftarrow 0 $\;
\For{$(d,d',c,y) \in \mathcal{B}$}{
$\overline{\textbf{m}}_{d}\leftarrow \textbf{Sample Representation}(\mathcal{G},d,s)$\;
$\overline{\textbf{m}}_{d'}\leftarrow \textbf{Sample Representation}(\mathcal{G},d',s)$\;
$\textbf{h}_{(d,d',c)}\leftarrow [\overline{\textbf{m}}_{d} \| \overline{\textbf{m}}_{d'} \|  \textbf{h}_{c}]$\;
$\hat{y}_{(d,d',c)} \leftarrow  f_{\Theta_H}(\textbf{h}_{(d,d',c)})$\;

$\mathcal{L} \leftarrow  \mathcal{L} + \ell(y; \hat{y}_{(d,d',c)})/|\mathcal{B}|$\;
}
}
		\caption{Mini-batch based forward pass of MOOMIN-A with approximate multi-scale multimodal representations.}\label{alg:batching}
	\end{algorithm}
\vspace{-5mm}



==> algorithms/sampling_algorithm.tex <==
	\begin{algorithm}[h!]
{\small		\DontPrintSemicolon
		\SetAlgoLined
		\KwData{$\mathcal{G}$ -- Bipartite drug -- protein interaction graph.\\
		$\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,d$ -- Source drug of interest.\\
		$\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,s$ -- Sample size.\\
		}
		\KwResult{$\overline{\textbf{m}}_d$ -- Sampled multi-scale representation of drug $\textit{d}.$}
$\widetilde{\textbf{m}}^0_d\leftarrow f_{\Theta_{D}}(\mathcal{M}_d)$\;
$\overline{\textbf{m}}_d\leftarrow\textbf{0}$\;
\For{$i \in \left \{1,\dots ,s\right \}$}{
$\widetilde{d}\leftarrow d$\;
$\widetilde{\textbf{m}}_d\leftarrow\widetilde{\textbf{m}}^0_d$\;
    \For{$l \in \left \{1,\dots ,r\right \}$}{
            \uIf{$l \mod 2 = 1$}{
            $\widetilde{p} \leftarrow \textbf{Random neighbor}(\mathcal{G}, \widetilde{d})$\;
            $\widetilde{\textbf{m}}^l_d \leftarrow f_{\Theta_p} (\textbf{x}_{\widetilde{p}}) $\;
            $\widetilde{\textbf{m}}_d \leftarrow [\widetilde{\textbf{m}}_d   \|  \widetilde{\textbf{m}}^l_d]$\;
            }
            \Else{
            $\widetilde{d} \leftarrow \textbf{Random neighbor}(\mathcal{G}, \widetilde{p})$\;
            $\widetilde{\textbf{m}}^l_{\widetilde{d}} \leftarrow f_{\Theta_D} (\mathcal{M}_d) $\;
            $\widetilde{\textbf{m}}_d \leftarrow [\widetilde{\textbf{m}}_d   \|  \widetilde{\textbf{m}}^l_d  ]$\;
            }
            }
            $\overline{\textbf{m}}_d \leftarrow \overline{\textbf{m}}_d + \widetilde{\textbf{m}}_d$ \;
}
            $\overline{\textbf{m}}_d \leftarrow \overline{\textbf{m}}_d /s$\;
}
		\caption{Approximate truncated random walk sampled multi-scale drug representation forward pass with MOOMIN.}\label{alg:sampling_algorithm}
	\end{algorithm}
	



==> figures/eyecandy.tex <==
\begin{figure}[h!]
\centering 
\includegraphics[scale=0.15]{./figures/moomin_text.jpg}
\caption{Given a pair of drugs (red and blue nodes) MOOMIN encodes drug representations using protein and compound structures that appear in the neighbourhood of the pair in an interaction graph. Using the representations its head layer predicts synergistic pairs which are effective at combating cancer.}
\end{figure}

==> figures/scales.tex <==
\begin{figure*}
\centering 
\includegraphics[scale=0.076]{./figures/scales_fun.jpg}
\caption{In this example the drug $d_3$ has a representation formed by concatenating aggregated drug and protein representations. These representation blocks at even scales $l=0,2,4$ are learned by aggregating the representations output by the drug-encoder using geometric properties of the compounds in the sets $\left\{d_1\right\},\left\{d_1;d_3\right\}$ and $\left\{d_1;d_2;d_3\right\}$. The odd scale representations at $l=1,3$ are learned by combining the protein representations generated by the protein encoder using the structural properties of the proteins in the sets $\left\{p_1\right\}$ and $\left\{p_1;p_2;p_3\right\}$.}\label{fig:main_explanation}
\end{figure*}

==> sections/0.abstract.tex <==
\begin{abstract}
In this report we present TigerLily a drug-drug interaction prediction system based on TigerGraph submitted to the Graph For All Million Dollar Challenge as a competition entry. Drug-drug interactions  
\end{abstract}

==> tables/molecule_size.tex <==
\begin{table}[h!]
\centering
\caption{The molecule and window size conditional test set performance of MOOMIN-E. We report average predictive performances calculated from 10 experimental runs with standard errors around the mean.}
\setlength{\tabcolsep}{4pt}
{\small
\begin{tabular}{ccccc}

%\cline{2-5}

 \textbf{Molecule Pair}&\textbf{Window}&\textbf{ROC AUC} &\textbf{PR AUC}  & \textbf{F}$_1$ \textbf{Score} \\
\hline
 &0&$.724\pm.007$ & $.767\pm .007$ & $.676 \pm .022$  \\
Large - Large &1&$\mathbf{.785\pm .007}$ & $\mathbf{.808\pm .008}$ & ${.733\pm .010}$  \\
 &2&${.763\pm .013}$ & ${.803\pm .008}$ & $\mathbf{.745\pm .006}$  \\
\hline
 &0&${.713\pm.005}$ & ${.656\pm .008}$ & ${.543 \pm .022}$  \\
Large - Small &1&$\mathbf{.778\pm .005}$ & ${.713\pm .008}$ & ${.656\pm .012}$  \\
 &2&${.768\pm .006}$ & $\mathbf{.717\pm .012}$ & $\mathbf{.678\pm .007}$  \\
\hline
 &0&${.614\pm .008}$ & ${.447\pm .011}$ & ${.312\pm .016}$  \\



Small - Small &1&${.715\pm .006}$ & ${.554\pm .010}$ & ${.477\pm .016}$  \\

 &2&$\mathbf{.716\pm .007}$ & $\mathbf{.563\pm .010}$ & $\mathbf{.516\pm .013}$  \\
%\hline
% &Large-Large&$\underset{\pm .048}{.751}$ & $\underset{\pm .026}{.802}$ & $\underset{\pm .078}{.734}$  \\
%3 &Large-Small&$\underset{\pm .033}{.764}$ & $\underset{\pm .034}{.721}$ & $\underset{\pm .074}{.673}$  \\
% &Small-Small&$\underset{\pm .027}{.713}$ & $\underset{\pm .032}{.570}$ & $\underset{\pm .067}{.508}$  \\
 \bottomrule
\end{tabular}}
\end{table}
\vspace{-5mm}

==> tables/multi_scale_models_related.tex <==
\begin{table}[h!]
\centering
\caption{A desiderata based comparison of MOOMIN and existing unsupervised and supervised multi-scale node representation learning algorithms.}\label{tab:related_multi}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
{\footnotesize
\begin{tabular}{ccccccc}
\toprule
\textbf{Method}&   \textbf{Implicit} & \textbf{Supervised} &\textbf{Attributed} & \textbf{Inductive} & \textbf{Multimodal}  \\
\hline 
 LINE \cite{tang2015line}& $\bullet$ &   &   &   &   \\
 GraRep \cite{cao2015grarep}&   &   &   &   &   \\
 Walklets \cite{perozzi2017don}&$\bullet$  &   &   &   &   \\
 MUSAE \cite{rozemberczki2019multi}& $\bullet$ &   & $\bullet$ &  &     \\
 \hline 
 FEATHER \cite{rozemberczki2020characteristic}& $\bullet$  & $\bullet$  & $\bullet$  &$\bullet$  &      \\
 MixHop \cite{abu2019mixhop}& $\bullet$  & $\bullet$  & $\bullet$  &$\bullet$  &      \\
SkipGNN \cite{huang2020skipgnn}&   & $\bullet$  & $\bullet$  &$\bullet$  &      \\
 HWGNN \cite{liu2019higher}& $\bullet$  & $\bullet$  & $\bullet$  &$\bullet$  &      \\
 SIGN \cite{rossi2020sign}& $\bullet$  &  $\bullet$ & $\bullet$  & $\bullet$ &       \\
 MOOMIN (ours) &$\bullet$  &$\bullet$  & $\bullet$ &$\bullet$ &$\bullet$     \\
\bottomrule
\end{tabular}
}
\end{table}
\vspace{-5mm}

==> tables/output_evidence.tex <==
\begin{table}[h!]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.2}
\caption{Out of sample drug combination predictions on (Vemurafenib, Drug, Cell line) triples that can be externally validated in the NCI Almanach \cite{holbeck2017national}.}\label{tab:samples}
\begin{tabular}{c c c c c ccc}
\toprule

\textbf{Drug A}&\textbf{Drug B}&  \textbf{Cell line}&\textbf{Tissue}& \textbf{Score}& \textbf{Label}\\ \hline
\multirow{7}{*}{Vemurafenib}&Cabazitaxel         &MDA-MB-435&breast&.831&synergy\\
&Pazopanib         &NCI-H522&lung&.803&synergy\\
&Crizotinib          &UO-31&kidney&.807&synergy\\
&Raloxifene   &SNB-75&brain&.860&synergy\\
&Axitnib      &MDA-MB-231&breast&.043&antagonism\\
&Carboplatin   &LOX IMVI&skin&.158&antagonism\\
&Chlorambucil        &SR&blood&.022&antagonism\\
\bottomrule
\end{tabular}


\end{table}

\vspace{-5mm}

==> tables/synergy_papers.tex <==
\begin{table}[h!]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\caption{A machine learning task, induction and input data type based comparison of MOOMIN and existing deep learning models that solve combination therapy problems.}\label{tab:related_drugs}
\begin{tabular}{@{} c c c cc cc }

& && \multicolumn{2}{c}{\textbf{Node Types}} & \multicolumn{2}{c}{\textbf{Node Features}}\\ \hline
\textbf{Method} &\textbf{Task}&\textbf{Inductive}&

\textbf{Drug}&\textbf{\,\,Protein\,}&

\textbf{Drug}&\textbf{\,\,Protein\,\,}\\

\hline
SkipGNN   \cite{huang2020skipgnn}      &Side Effect        &&$\bullet$&  &&\\
DECAGON   \cite{zitnik2018modeling}    &Side Effect         &&$\bullet$&$\bullet$&&\\
ESP       \cite{burkhardt2019esp}      &Side Effect        &&$\bullet$&$\bullet$ &&\\
TIP       \cite{xu2020tip}             &Side Effect        &&$\bullet$&$\bullet$ &&\\
DeepDDI   \cite{ryu2018deep}       &Side Effect       &&$\bullet$&              &$\bullet$&\\
SumGNN \cite{yu2021sumgnn}       &Side Effect   &&$\bullet$&$\bullet$ &$\bullet$&\\
\hline
DeepCCI   \cite{kwon2017deepcci}       &Interaction        &$\bullet$&&&           $\bullet$&\\
MR-GNN   \cite{xu2019mr}       &Interaction        &$\bullet$&&&                   $\bullet$&\\
\hline
DrugCell  \cite{kuenzi2020predicting}  &Synergy &$\bullet$&&$\bullet$  &$\bullet$&\\
DeepSynergy   \cite{preuer2018deepsynergy}       &Synergy        &$\bullet$&&     &$\bullet$&\\
MOOMIN (ours)   &Synergy        &$\bullet$&$\bullet$&$\bullet$&           $\bullet$&$\bullet$\\
\bottomrule
\end{tabular}


\end{table}
\vspace{-5mm}
